Exploring & Exploiting High-Order Graph Structure for Sparse Knowledge Graph Completion

Sparse knowledge graph (KG) scenarios pose a challenge for previous Knowledge Graph Completion (KGC) methods, that is, the completion performance decreases rapidly with the increase of graph sparsity. This problem is also exacerbated because of the widespread existence of sparse KGs in practical applications. To alleviate this challenge, we present a novel framework, LR-GCN, that is able to automatically capture valuable long-range dependency among entities to supplement insufficient structure features and distill logical reasoning knowledge for sparse KGC. The proposed approach comprises two main components: a GNN-based predictor and a reasoning path distiller. The reasoning path distiller explores high-order graph structures such as reasoning paths and encodes them as rich-semantic edges, explicitly compositing long-range dependencies into the predictor. This step also plays an essential role in densifying KGs, effectively alleviating the sparse issue. Furthermore, the path distiller further distills logical reasoning knowledge from these mined reasoning paths into the predictor. These two components are jointly optimized using a well-designed variational EM algorithm. Extensive experiments and analyses on four sparse benchmarks demonstrate the effectiveness of our proposed method.

==> Images/architecture.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/framework_1.pdf}
    \caption{Our framework consists of two modules: GNN-based model with the long range dependency convolution layer and MLN-RL model, which are jointly optimized by high-order knowledge distillation. Given a query $(e_s,r_q,?)$, MLN-RL first reasons paths and classify the paths into two parts according to whether the path is correct. The positive paths and negative path segments are applied to construct new edges to capture long range dependency explicitly. While the negative paths are fed into MLN to distill knowledge for the GNN-based model by variational EM algorithm.} 
    % (todo: 1. colors are not that powerful. 2. not highlight what is high-order structures. 3. ensure the clarity of high-level idea and each component, then add details. )}
    \label{fig:architecture}
\end{figure*}

==> Images/case_studies.tex <==
% \begin{figure*}[htbp]
% 	\centering
% 	\subfloat[a]{\includegraphics[width=.8\linewidth]{Figures/case studies_1.pdf}}\\
% 	\subfloat[b]{\includegraphics[width=.8\linewidth]{Figures/case studies_2.pdf}}\\
%     \subfloat[c]{\includegraphics[width=.8\linewidth]{Figures/case studies_3.pdf}}\\
% 	\caption{Case studies.}
% \end{figure*}

\begin{figure*}[t]
	\centering
	\subfigure[Case 1: (\textit{Intelligent dance music, parent\_genre, ?})]{
		\begin{minipage}{14cm}%[b]%{0.2\textwidth}
			\includegraphics[width=\textwidth]{Figures/case_studies_2.pdf} \\
			
		\end{minipage}
	}
    \subfigure[Case 2: (\textit{David Nutter, nominated\_for, ?})]{
		\begin{minipage}{14cm} %[b]%{0.2\textwidth} 
                        %{12cm or 0.2/textwidth} 控制图片大小，可以=textwidth
			% 插入子图片
                        \includegraphics[width=\textwidth]{Figures/case_studies_3.pdf} \\
			%\includegraphics[width=\textwidth]{fig/beforePAA.eps} 
                        % 可以在一个minipage里写多张图片，它们共用一个小标题\subfigure['sub_title']
		\end{minipage}
	}
    \caption{Blue edges denote the reasoning paths searched for corresponding queries. Orange and green nodes denote the predicted answers by the pre-trained GNN-based predictor before joint learning and the golden answers, respectively.}
    \label{fig:case_study}
\end{figure*}

==> Images/decrease_trend.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/decrease_trend.pdf}
    \caption{KGC results of different previous KG embedding models on FB15K-237 and its sparse subsets (60\%, 40\%, and 20\% denote percentages of retained triples). The performance drops dramatically as we remove triples.}
    \label{fig:decrease_trend}
\end{figure}

==> Images/in-degree_analysis.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/in-degree_analysis.pdf}
    \caption{MRR results and entity frequency grouped by entity in-degree on NELL23K and FB15K-237\_10.}
    \label{fig:in-degree_analysis}
\end{figure}

==> Images/path_induce_rule.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/path_induce_rule.pdf}
    \caption{An illustration of inducing rules from reasoning paths. To reduce the length of rules, we view loops within paths as pointless segments and remove them.}
    \label{fig:path_induce_rule}
\end{figure}

==> Images/path_use_example.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/using_path_example.pdf}
    \caption{The sample illustration of how to utilize true-prediction paths and false-prediction paths, respectively. More details please refer to Section 3. (todo: true/false lack definition, very confusing. )}
    \label{fig:handle_path_example}
\end{figure}

==> Images/sparsity_analysis.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/sparsity_analysis.pdf}
    \caption{Improvements of LR-GCN on FB15K-237 and 4 sparse datasets against to CompGCN (60\%, 30\%, 20\%, and 10\% denote percentages of retained triples).}
    \label{fig:sparsity_analysis}
\end{figure}

==> Tables/case_study.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c} %表格7列 全部居中显示
        \hline
        \hline
        Queries & Answer & CompGCN & MultihopKG & LR-GCN \\
        \hline
        (Haim Saban, nationality, ?) & USA & Actor-GB & \makecell{(Haim Saban, program, Mighty Morphin Power Rangers)\\ $\wedge$(Mighty Morphin Power Rangers, country\_of\_origin, USA)} & USA \\
        \hline
        \makecell{(14th Screen Actors Guild Awards, \\award\_winner, ?)} & Edie Falco & Ernest Hemingway & \makecell{(14th Screen Actors Guild Awards, award\_winner, \\Matt Servitto)$\wedge$(Matt Servitto, award\_winner, Edie Falco)\\$\wedge$(Edie Falco, award\_nominee, Dan Grimaldi)} & Edie Falco \\
        \hline
        % (Orange County, film\_crew\_role, ?) & \makecell{Special Effects \\Supervisor} & \makecell{Special Effects \\Supervisor} & \makecell{(Orange County, category, Official Website)\\ \wedge(Official Website, category_inv, Ghost World)\\ \wedge
        % (Ghost World, film_crew_role, Visual Effects Supervisor)} & \makecell{2,(beautiful, \underline{fun}, cool, \\ colorful, expensive)} \\
    \end{tabular}
    }
    \caption{Two cases from FB15K-237\_10. The first column includes queries, on which CompGCN fails to predict correctly, while LR-GCN predicts truly with the explicit modeling of reasoning paths from MultihopKG.}
    \label{tab:case_studies}
\end{table*}

==> Tables/dataset_statistics.tex <==
% \begin{table*}[t]
%     \centering
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{l|cccccccc}
%     \toprule
%      & WD-singer & NELL23K & FB15K-237\_10 & FB15K-237\_20 & FB15K-237\_30 & FB15K-237\_40 & FB15K-237\_60 & FB15K-237 \\
%     \midrule
%     \#Entity & 10282 & 22925 & 14541 & 14541 & 14541 & 14541 & 14541 & 14541 \\
%     \#Relation & 270 & 400 & 237 & 237 & 237 & 237 & 237 & 237 \\
%     \#Train Set & 16142 & 24321 & 27211 & 54423 & 81634 & 108846 & 163269 & 272115 \\
%     \#Dev Set & 2163 & 4951 & 17535 & 17535 & 17535 & 17535 & 17535 & 17535 \\
%     \#Test Set & 2203 & 4944 & 20466 & 20466 & 20466 & 20466 & 20466 & 20466 \\
%     Average Out Degree & 1.570 & 1.170 & 1.876 & 3.752 & 5.628 & 7.504 & 11.256 & 18.760\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Summary statistics of datasets}
%     \label{tab:dataset_statistics}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Summary statistics of datasets}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccccccc}
    \toprule
     & WD-singer & NELL23K & FB15K-237\_10 & FB15K-237\_20 & FB15K-237\_30 & FB15K-237\_60 & FB15K-237 \\
    \midrule
    \#Entity & 10282 & 22925 & 14541 & 14541 & 14541 & 14541 & 14541 \\
    \#Relation & 270 & 400 & 237 & 237 & 237 & 237 & 237 \\
    \#Train Set & 16142 & 24321 & 27211 & 54423 & 108846 & 163269 & 272115 \\
    \#Dev Set & 2163 & 4951 & 17535 & 17535 & 17535 & 17535 & 17535 \\
    \#Test Set & 2203 & 4944 & 20466 & 20466 & 20466 & 20466 & 20466 \\
    Avg In-degree & 1.570 & 1.170 & 1.876 & 3.752 & 5.628 & 11.256 & 18.760\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:dataset_statistics}
\end{table*}

==> Tables/hyperparameter_influence.tex <==
\begin{table}[htbp]
    \centering
    % \resizebox{\linewidth}{!}{
    \begin{subtable}[t]{0.45\linewidth}
        \begin{tabular}{cccccccc}
            \toprule
            && \multicolumn{6}$\gamma$\\
            \cmidrule(lr){3-8}
            && 0.5 & 1.0 & 2.0 & 3.0 & 4.0 & 5.0\\
            \midrule
            \multirow{3}*{$\beta$} & 0.1 & - & 24.12 & \underline{24.96} & 24.64 & - & -\\
            ~ & 0.5 & 23.94 & 24.38 & \textbf{25.27} & 24.80 & 24.7 & 24.58\\
            ~ & 1.0 & 23.73 & 23.99 & 24.52 & 24.21 & - & -\\
            \bottomrule
        \end{tabular}
        % }
        \caption{NELL23K.}
    \end{subtable}

    \begin{subtable}[t]{0.45\linewidth}
        \begin{tabular}{cccccc}
            \toprule
            && \multicolumn{4}$\gamma$\\
            \cmidrule(lr){3-6}
            && 2.0 & 3.0 & 4.0 & 5.0\\
            \midrule
            \multirow{4}*{$\beta$} & 0.1 & - & 16.38 & - & \underline{16.47}\\
            ~ & 0.5 & - & 16.37 & 16.39 & 16.35\\
            ~ & 1.0 & 16.17 & 16.31 & 16.37 & \textbf{16.49}\\
            ~ & 2.0 & 16.15 & 16.16 & 16.19 & -\\
            \bottomrule
        \end{tabular}
        % }
        \caption{FB15K-237\_10.}
    \end{subtable}
    \caption{Influences of $\beta$ and $\gamma$ on NELL23K and FB15K-237\_10.}
    \label{tab:hyperparameter_influence}
\end{table}

% \begin{table}[htbp]
%     \centering
%     % \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccc}
%         \toprule
%         && \multicolumn{4}$\gamma$\\
%         \cmidrule(lr){3-6}
%         && 2.0 & 3.0 & 4.0 & 5.0\\
%         \midrule
%         \multirow{4}*{$\beta$} & 0.1 & - & 16.38 & - & \underline{16.47}\\
%         ~ & 0.5 & - & 16.37 & 16.39 & 16.35\\
%         ~ & 1.0 & 16.17 & 16.31 & 16.37 & \textbf{16.49}\\
%         ~ & 2.0 & 16.15 & 16.16 & 16.19 & -\\
%         \bottomrule
%     \end{tabular}
%     % }
%     \caption{Influences of $\beta$ and $\gamma$ on FB15K-237\_10.}
%     \label{tab:hyperparameter_influence_fb}
% \end{table}

==> Tables/hyperparameters.tex <==
\begin{table}[htbp]
    \centering
    \caption{Part of best hyperparameter settings and running time of LR-GCN for different datasets. ``TT" means ``Training time".}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    && $\beta$ & $\gamma$ & $\lambda$ & TT\\
    \midrule
    \multicolumn{2}{l}{FB15K-237\_10} & 1.0 & 5.0 & 0.0 & 4h\\
    \multicolumn{2}{l}{FB15K-237\_20} & 2.0 & 5.0 & 0.0001 & 13.5h\\
    \multicolumn{2}{l}{FB15K-237\_30} & 1.0 & 1.0 & 0.001 & 12.5h\\
    \multicolumn{2}{l}{FB15K-237\_60} & 2.0 & 0.1 & 0.0 & 15.5h\\
    \multicolumn{2}{l}{WD-singer} & 1.0 & 1.0 & 0.001 & 9h\\
    \multicolumn{2}{l}{NELL23K} & 0.5 & 2.0 & 0.0 & 2h\\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:hyperparameters}
\end{table}

==> Tables/k_stack.tex <==
\begin{table}[t]
    \centering
    \caption{Performance comparison of LR-GCN with CompGCN stacked with $K=1,2,3$ graph convolutional layers on WD-singer and NELL23K.}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    && \multicolumn{2}{c}{WD-singer} & \multicolumn{2}{c}{NELL23K}\\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    && Hits@10 & MRR & Hits@10 & MRR\\
    \midrule
    \multicolumn{2}{l}{CompGCN(K=1)} & 47.62 & 37.65 & 37.57 & 21.60\\
    \multicolumn{2}{l}{CompGCN(K=2)} & 47.98 & 36.55 & 37.34 & 21.13\\
    \multicolumn{2}{l}{CompGCN(K=3)} & 47.80 & 34.22 & 37.55 & 21.01\\
    \multicolumn{2}{l}{LR-GCN} & \textbf{49.98} & \textbf{39.27} & \textbf{41.90} & \textbf{25.27}\\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:k_stack}
\end{table}


% \begin{minipage}{\textwidth}
%     \begin{minipage}[htbp]{0.4\textwidth}
%         \centering
%         \makeatletter\def\@captype{table}\makeatother
%         \begin{tabular}{cccccc}
%         \toprule
%         && \multicolumn{2}{c}{WD-singer} & \multicolumn{2}{c}{NELL23K}\\
%         \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%         && Hits@10 & MRR & Hits@10 & MRR\\
%         \midrule
%         \multicolumn{2}{l}{CompGCN(K=1)} & 47.62 & 37.65 & 37.57 & 21.60\\
%         \multicolumn{2}{l}{CompGCN(K=2)} & 47.98 & 36.55 & 37.34 & 21.13\\
%         \multicolumn{2}{l}{CompGCN(K=3)} & 47.80 & 34.22 & 37.55 & 21.01\\
%         \multicolumn{2}{l}{LR-GCN} & \textbf{49.98} & \textbf{39.27} & \textbf{41.90} & \textbf{25.27}\\
%         \bottomrule
%         \end{tabular}
%         \caption{Performance comparison of LR-GCN with CompGCN stacked with $K=1,2,3$ graph convolutional layers on WD-singer and NELL23K.}
%     \end{minipage}
    
%     \begin{minipage}[htbp]{0.45\textwidth}
%         \centering
%         \makeatletter\def\@captype{table}\makeatother
%         \begin{tabular}{ccc}
%         \hline
%         n  & L  & $L+n$ \\ \hline
%         0  & 1  & 1 \\
%         1  & 3  & 4 \\
%         2  & 5  & 7 \\
%         3  & 7  & 10\\
%         4  & 9  & 13 \\
%         5  & 11 & 16 \\
%         \hline
%         \end{tabular}
%         \caption{title2}
%     \end{minipage}
% \end{minipage}


% \begin{table}
%     \centering
% 	\begin{minipage}{0.35\linewidth}
% 		\centering
%         \begin{tabular}{cccccc}
%         \toprule
%         && \multicolumn{2}{c}{WD-singer} & \multicolumn{2}{c}{NELL23K}\\
%         \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%         && Hits@10 & MRR & Hits@10 & MRR\\
%         \midrule
%         \multicolumn{2}{l}{CompGCN(K=1)} & 47.62 & 37.65 & 37.57 & 21.60\\
%         \multicolumn{2}{l}{CompGCN(K=2)} & 47.98 & 36.55 & 37.34 & 21.13\\
%         \multicolumn{2}{l}{CompGCN(K=3)} & 47.80 & 34.22 & 37.55 & 21.01\\
%         \multicolumn{2}{l}{LR-GCN} & \textbf{49.98} & \textbf{39.27} & \textbf{41.90} & \textbf{25.27}\\
%         \bottomrule
%         \end{tabular}
%         \caption{The crane}
%         \label{table:NormalSafe}
% 	\end{minipage}
% 	%\qquad
% 	\hfill
% 	\begin{minipage}{0.4\linewidth}
% 		\centering
%         \begin{tabular}{cccccc}
%         \toprule
%         && \multicolumn{2}{c}{DacKGR} & \multicolumn{2}{c}{MLN-RL}\\
%         \cmidrule(lr){3-4}\cmidrule(lr){5-6}
%         && Hits@1 & MRR & Hits@1 & MRR\\
%         \midrule
%         \multicolumn{2}{l}{FB15K-237\_10} & 10.21 & 13.91 & 10.33 & 13.97\\
%         \multicolumn{2}{l}{WD-singer} & 26.49 & 32.66 & 28.05 & 33.65\\
%         \multicolumn{2}{l}{NELL23K} & 13.00 & 18.99 & 13.02 & 19.05\\
%         \bottomrule
%         \end{tabular}
%         \caption{The crane}
%         \label{table:NormalSafe}
% 	    \end{minipage}
% \end{table}

==> Tables/main_results.tex <==
% \begin{table*}[t]
%     \centering
%     % \small
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cccccccccccccccc}
%     \toprule
%     &&&& \multicolumn{3}{c}{FB15K-237\_{10}} & \multicolumn{3}{c}{FB15K-237\_{20}} & \multicolumn{3}{c}{WD-singer} & \multicolumn{3}{c}{NELL23K}\\
%     \cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
%     &&&& \multicolumn{2}{c}{Hits@N $\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$}\\
%     \cmidrule(lr){5-6}\cmidrule(lr){8-9}\cmidrule(lr){11-12}\cmidrule(lr){14-15}
%     &&&& @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$\\
%     \midrule
%     \multicolumn{4}{l}{TransE \cite{bordes2013translating}} & 4.94 & 24.03 & 11.58 & 8.33 & 28.76 & 15.27 & 22.56 & \underline{49.84} & 32.68 & 4.62 & 30.21 & 13.35\\
%     \multicolumn{4}{l}{RotatE \cite{sun2019rotate}} & 5.64 & 17.16 & 9.52 & 10.40 & 28.52 & 16.43 & 31.43 & 45.96 & 36.79 & 9.63 & 28.13 & 15.75\\
%     \multicolumn{4}{l}{DistMult \cite{balavzevic2019tucker}} & 9.51 & 22.85 & 13.90 & 10.68 & 26.72 & 15.92 & 25.51 & 39.51 & 30.63 & 12.71 & 33.26 & 19.50\\
%     \multicolumn{4}{l}{ComplEx \cite{trouillon2016complex}} & 9.61 & 22.77 & 13.92 & 10.69 & 26.17 & 15.81 & 29.87 & 43.53 & 34.94 & 14.21 & 32.57 & 20.26\\
%     \multicolumn{4}{l}{TuckER \cite{balavzevic2019tucker}} & 6.51 & 16.44 & 9.89 & 9.73 & 25.91 & 15.08 & 32.12 & 44.83 & 36.87 & 13.75 & 30.35 & 19.36\\
%     \multicolumn{4}{l}{ConvE \cite{dettmers2018convolutional}} & 10.56 & 23.90 & 15.69 & 11.38 & 29.51 & 17.27 & 31.46 & 47.37 & 37.22 & 14.44 & 37.55 & 22.73\\
%     \multicolumn{4}{l}{SACN \cite{shang2019end}} & - & - & - & - & - & - & - & - & - & - & - & -\\
%     \multicolumn{4}{l}{DacKGR \cite{lv2020dynamic}} & 10.21 & 21.34 & 13.91 & 10.99 & 26.15 & 15.87 & 26.49 & 44.30 & 32.66 & 13.00 & 31.63 & 18.99\\
%     % \multicolumn{4}{l}{KBGAT} & - & - & - & - & - & - & - & - & - & - & - & -\\
%     \midrule
%     \multicolumn{4}{l}{CompGCN \cite{vashishth2019composition}} & 9.52 & 23.11 & 14.11 & 11.27 & 29.51 & 17.30 & 31.75 & 47.62 & 37.65 & 13.79 & 37.57 & 21.59\\
%     \midrule
%     \multicolumn{4}{l}{LR-GCN (w/o KD)} & 10.41 & \underline{26.32} & 15.77 & \underline{11.94} & \underline{30.98} & \underline{18.22} & \underline{32.06} & 49.61 & \underline{38.71} & 15.41 & \underline{39.84} & 23.41\\
%     % \multicolumn{4}{l}{\textit{–Impr}} & () & () & () & () & () & () & () & () & () & () & () & ()\\
%     \multicolumn{4}{l}{LR-GCN (w/o LRC)} & \underline{10.60} & 26.25 & \underline{15.89} & 11.59 & 30.11 & 17.74 & 31.89 & 48.28 & 38.00 & \underline{15.99} & 39.11 & \underline{23.53}\\
%     % \multicolumn{4}{l}{\textit{–Impr}} & () & () & () & () & () & () & () & () & () & () & () & ()\\
%     \multicolumn{4}{l}{LR-GCN} & \textbf{10.81} & \textbf{26.68} & \textbf{16.12} & \textbf{12.15} & \textbf{31.14} & \textbf{18.45} & \textbf{32.46} & \textbf{50.09} & \textbf{39.02} & \textbf{16.68} & \textbf{41.31} & \textbf{24.68}\\
%     \multicolumn{4}{l}{\textit{–Rela. Impr.}} & +\textit{13.55\%} & +\textit{15.45\%} & +\textit{14.25\%} & +\textit{7.81\%} & +\textit{5.52\%} & +\textit{6.65\%} & +\textit{2.24\%} & +\textit{5.19\%} & +\textit{3.64\%} & +\textit{9.21\%} & +\textit{9.95\%} & +\textit{14.31\%}\\
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Experimental results on FB15K-237\_10, FB15K-237\_20, WD-singer, and NELL23K. The last line records the relative improvements of LR-GCN over CompGCN. Hits@N and MRR values are in percentage. ``KD" denotes High-order Knowledge Distillation and ``LRC" represents Long Range Convolution. The best score is in \textbf{bold} and the second is \underline{underlined}.}
%     \label{tab:main_results}
% \end{table*}

\begin{table*}[t]
    \centering
    \caption{Experimental results on FB15K-237\_10, FB15K-237\_20, WD-singer, and NELL23K. The last line records the relative improvements of LR-GCN over CompGCN. Hits@N and MRR values are in percentage. ``KD" denotes High-order Knowledge Distillation and ``LRC" represents Long Range Convolution. The best score is in \textbf{bold} and the second is \underline{underlined}.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccccccccccccc}
    \toprule
    &&&& \multicolumn{3}{c}{FB15K-237\_{10}} & \multicolumn{3}{c}{FB15K-237\_{20}} & \multicolumn{3}{c}{WD-singer} & \multicolumn{3}{c}{NELL23K}\\
    \cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}\cmidrule(lr){14-16}
    &&&& \multicolumn{2}{c}{Hits@N $\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$} && \multicolumn{2}{c}{Hits@N$\uparrow$}\\
    \cmidrule(lr){5-6}\cmidrule(lr){8-9}\cmidrule(lr){11-12}\cmidrule(lr){14-15}
    &&&& @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$ & @1 & @10 & MRR $\uparrow$\\
    \midrule
    \multicolumn{4}{l}{TransE} & 4.94 & 24.03 & 11.58 & 8.33 & 28.76 & 15.27 & 22.56 & \underline{49.84} & 32.68 & 4.62 & 30.21 & 13.35\\
    \multicolumn{4}{l}{RotatE} & 5.64 & 17.16 & 9.52 & 10.40 & 28.52 & 16.43 & 31.43 & 45.96 & 36.79 & 9.63 & 28.13 & 15.75\\
    % \multicolumn{4}{l}{DistMult} & 9.51 & 22.85 & 13.90 & 10.68 & 26.72 & 15.92 & 25.51 & 39.51 & 30.63 & 12.71 & 33.26 & 19.50\\
    \multicolumn{4}{l}{ComplEx} & 9.61 & 22.77 & 13.92 & 10.69 & 26.17 & 15.81 & 29.87 & 43.53 & 34.94 & 14.21 & 32.57 & 20.26\\
    \multicolumn{4}{l}{TuckER} & 6.51 & 16.44 & 9.89 & 9.73 & 25.91 & 15.08 & 32.12 & 44.83 & 36.87 & 13.75 & 30.35 & 19.36\\
    \multicolumn{4}{l}{ConvE} & 10.56 & 23.90 & 15.69 & 11.38 & 29.51 & 17.27 & 31.46 & 47.37 & 37.22 & 14.44 & 37.55 & 22.73\\
    \multicolumn{4}{l}{SACN} & 9.60 & 22.56 & 13.98 & 11.36 & 28.82 & 17.07 & 28.49 & 43.70 & 34.10 & 14.36 & 35.01 & 21.22\\
    \multicolumn{4}{l}{RED-GNN} & 8.43 & 19.8 & 12.22 & {12.28} & 30.88 & {18.43} & {32.57} & 49.18 & {38.79} & \underline{16.63} & 39.65 & {24.24} \\
    \multicolumn{4}{l}{NBFNet} & \textbf{11.13} & \textbf{27.78} & \textbf{16.64} & \underline{12.45} & \textbf{31.87} & \underline{18.89} & \underline{32.59} & 48.10 & {38.81} & {14.40} & 39.04 & {22.74} \\
    \midrule
    \multicolumn{4}{l}{DacKGR} & 10.21 & 21.34 & 13.91 & 10.99 & 26.15 & 15.87 & 26.49 & 44.30 & 32.66 & 13.00 & 31.63 & 18.99\\
     \multicolumn{4}{l}{HoGRN} & - & - & - & - & - & - & - & 48.80 & \underline{39.07} & - & \underline{39.98} & \underline{24.56}\\
    % \multicolumn{4}{l}{KBGAT} & - & - & - & - & - & - & - & - & - & - & - & -\\
    \midrule
    \multicolumn{4}{l}{\textit{-backbone}}\\
    \multicolumn{4}{l}{CompGCN} & 9.52 & 23.11 & 14.11 & 11.27 & 29.51 & 17.30 & 31.75 & 47.62 & 37.65 & 13.79 & 37.57 & 21.59\\
    \midrule
    \multicolumn{4}{l}{LR-GCN (w/o KD)} & 10.41 & {26.32} & 15.77 & {11.94} & {30.98} & {18.22} & {32.06} & 49.61 & {38.71} & 15.41 & {39.84} & 23.41\\
    % \multicolumn{4}{l}{\textit{–Impr}} & () & () & () & () & () & () & () & () & () & () & () & ()\\
    \multicolumn{4}{l}{LR-GCN (w/o LRC)} & {10.60} & 26.25 & {15.89} & 11.59 & 30.11 & 17.74 & 31.89 & 48.28 & 38.00 & {15.99} & 39.11 & {23.53}\\
    % \multicolumn{4}{l}{\textit{–Impr}} & () & () & () & () & () & () & () & () & () & () & () & ()\\
    \multicolumn{4}{l}{LR-GCN} & \underline{11.07} & \underline{27.37} & \underline{16.49} & \textbf{12.57} & \underline{31.72} & \textbf{18.97} & \textbf{32.80} & \textbf{49.98} & \textbf{39.27} & \textbf{17.31} & \textbf{41.90} & \textbf{25.27}\\
    \multicolumn{4}{l}{\textit{–Rela. Impr.}} & +\textit{16.28\%} & +\textit{18.43\%} & +\textit{16.87\%} & +\textit{11.54\%} & +\textit{7.49\%} & +\textit{9.65\%} & +\textit{3.31\%} & +\textit{4.96\%} & +\textit{5.50\%} & +\textit{25.53\%} & +\textit{11.53\%} & +\textit{17.04\%}\\
    \bottomrule
    \end{tabular}
    }
    \label{tab:main_results}
\end{table*}

==> Tables/mln_rl.tex <==
\begin{table}[t]
    \centering
    \caption{Performances of MLN-RL compared with its base model DacKGR on FB15K-237\_10, WD-singer and NELL23K. Values are in percentage.}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{cccccc}
    \toprule
    && \multicolumn{2}{c}{DacKGR} & \multicolumn{2}{c}{MLN-RL}\\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    && Hits@1 & MRR & Hits@1 & MRR\\
    \midrule
    \multicolumn{2}{l}{FB15K-237\_10} & 10.21 & 13.91 & 10.33 & 13.97\\
    \multicolumn{2}{l}{WD-singer} & 26.49 & 32.66 & 28.05 & 33.65\\
    \multicolumn{2}{l}{NELL23K} & 13.00 & 18.99 & 13.02 & 19.05\\
    \bottomrule
    \end{tabular}
    % }
    \label{tab:mln_performance}
\end{table}
